Optimization at the Interface of Unitary and Non-unitary Quantum Operations in PCOAST

The Pauli-based Circuit Optimization, Analysis and Synthesis Toolchain (PCOAST) was recently introduced as a framework for optimizing quantum circuits. It converts a quantum circuit to a Pauli-based graph representation and provides a set of optimization subroutines to manipulate that internal representation as well as methods for re-synthesizing back to a quantum circuit. In this paper, we focus on the set of subroutines which look to optimize the PCOAST graph in cases involving unitary and non-unitary operations as represented by nodes in the graph. This includes reduction of node cost and node number in the presence of preparation nodes, reduction of cost for Clifford operations in the presence of preparations, and measurement cost reduction using Clifford operations and the classical remapping of measurement outcomes. These routines can also be combined to amplify their effectiveness. We evaluate the PCOAST optimization subroutines using the Intel Quantum SDK on examples of the Variational Quantum Eigensolver (VQE) algorithm. This includes synthesizing a circuit for the simultaneous measurement of a mutually commuting set of Pauli operators. We find for such measurement circuits the overall average ratio of the maximum theoretical number of two-qubit gates to the actual number of two-qubit gates used by our method to be 7.91.

==> src/Figures/opt_ex2.tex <==
\begin{figure*} \label{fig:opt}
\centering
   
   \begin{tikzpicture}
     \node[scale=0.7]{
       \begin{tikzcd}[row sep=0.2cm]
           &\startingpoprgate{\Meas[c_0]{Y_0 X_1 Z_2}} \arrow[rd]
         \\
         \startingpoprgate{\Prep{X_0}{Y_0}} \arrow[r] \arrow[rd] \arrow[ru]
         &\poprgate{\Rot{Z_0 Z_1}{\theta_1}} \arrow[r]
         & \startingframegate{1}{\begin{pmatrix}
                Z_0 X_1 & Z_1 \\
                Z_0 & X_0 Z_1 \\
                Z_2 & X_2
           \end{pmatrix}}
         \\
         &\startingpoprgate{\Meas[c_1]{X_0 Y_1 Z_2}} \arrow[ru]
         %\\
         %&\startingpoprgate{\Meas[c_1]{Z_2}}
       \end{tikzcd}
     };

     \node at (4.75, 0) {\Large $\underset{(\text{mod }{c_0 \otimes c_1})}{\simeq}$ };

     \node[scale=0.7] at (9, 0) {
       \begin{tikzcd}[row sep=0.2cm]
           &\startingpoprgate{\Meas[c_0]{Y_0 X_1 Z_2}} \arrow[rd]
         \\
         \poprgate{\Prep{X_0}{Y_0}} \arrow[rd] \arrow[ru]
         &
           & \startingframegate{1}{\begin{pmatrix}
                Z_0 & X_0 \\
                Z_1 & X_1 \\
                Z_2 & X_2
           \end{pmatrix}}
         \\
         &\startingpoprgate{\Meas[c_1]{X_0 Y_1 Z_2}} \arrow[ru]
       \end{tikzcd}
     };

     \node at (4.75, -1.5) {\Large $\underset{(\text{mod }{c_0 \otimes c_1})}{\simeq}$ };

     \node[scale=0.7] at (0, -3) {
       \begin{tikzcd}[row sep=0.2cm]
           & &\startingpoprgate{\Meas[c_0]{Y_0}}
         \\
         \poprgate{\Prep{X_0}{Y_0}} \arrow[r]
         & \startingframegate{1}{\begin{pmatrix}
                Z_0 X_1 & X_0 \\
                Z_1 X_0 & X_1 \\
                Z_2 & X_2
           \end{pmatrix}} \arrow[ru] \arrow[rd]
         &\startingpoprgate{\Meas[c_0 + c_1]{Z_2}}
         \\
         & &\startingpoprgate{\Meas[c_1]{Y_1}}
       \end{tikzcd}
     };

     \node at (4.75, -3) {\Large $\underset{(\text{mod }{c_0 \otimes c_1})}{\simeq}$ };

%     \node[scale=0.7] at (0, -10.5) {
%       \begin{tikzcd}[row sep=0.2cm]
%           & &\startingpoprgate{\Meas[c_0]{Y_0}}
%         \\
%        \poprgate{\Prep{X_0}{Y_0}} \arrow[r]
%         & \startingframegate{1}{\begin{pmatrix}
%                Y_0 & X_0 \\
%                Z_1 & X_1 \\
%                Z_2 & X_2
%           \end{pmatrix}} \arrow[ru]
%         &\startingpoprgate{\Meas[c_0 + c_1 + c_2]{Z_2}}
%         \\
%         & &\startingpoprgate{\Meas[c_2]{Y_1}}
%       \end{tikzcd}
%     };

%     \node at (0, -12.25) {\Large $\simeq (\mod c_0 \otimes c_1$) };
% prev -14
     \node[scale=0.7] at (9, -3) {
       \begin{tikzcd}[row sep=0.2cm]
           &\startingpoprgate{\Meas[c_0]{-Z_0}}
         \\
         \poprgate{\Prep{X_0}{Y_0}} \arrow[ru]
         &\startingpoprgate{\Meas[c_0 + c_1 + c_2]{Z_2}}
           & \startingframegate{1}{\begin{pmatrix}
                Z_0 & X_1 \\
                Z_1 & X_1 \\
                Z_2 & X_2
           \end{pmatrix}}
         \\
         &\startingpoprgate{\Meas[c_2]{Y_1}}
       \end{tikzcd}
     };
     
    \end{tikzpicture}

    \caption{blaga}
  
\end{figure*}

==> src/Tables/n_meas.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{Statistics for the measurement circuits for each molecule's for both BK and JW mappings.}
\label{tab:n_meas}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccccccccc@{}}
\toprule
\multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{2}{c}{Avg total gates} &
  \multicolumn{2}{c}{Avg 2Q gates} &
  \multicolumn{2}{c}{Avg Depth} &
  \multicolumn{2}{c}{Avg $r_{2q}$} &
  \multicolumn{2}{c}{Avg $k$} \\ \cmidrule(l){5-14} 
Benchmark & \# Qubits & \# Messurements & \# Groupings & BK    & JW    & BK    & JW    & BK    & JW    & BK    & JW    & BK    & JW    \\ \midrule
H2        & 4         & 15              & 2            & 5.00  & 12.00 & 0.00  & 2.50  & 1.50  & 4.50  & -     & 2.40  & 4.00  & 3.50  \\
HF        & 12        & 631             & 38           & 41.61 & 38.34 & 9.79  & 8.89  & 10.53 & 7.89  & 6.53  & 7.12  & 10.26 & 9.82  \\
LiH       & 12        & 631             & 41           & 38.07 & 36.34 & 8.27  & 8.34  & 9.41  & 8.15  & 7.76  & 7.24  & 10.46 & 9.54  \\
BeH2      & 14        & 666             & 36           & 47.33 & 43.83 & 11.47 & 10.36 & 11.17 & 9.69  & 7.53  & 8.40  & 11.31 & 11.31 \\
H2O       & 14        & 1086            & 50           & 48.98 & 46.88 & 11.52 & 11.46 & 10.76 & 9.78  & 7.65  & 7.58  & 11.98 & 11.36 \\
BH3       & 16        & 1957            & 76           & 48.85 & 53.15 & 10.29 & 13.11 & 10.45 & 10.03 & 11.47 & 8.93  & 14.40 & 13.57 \\
NH3       & 16        & 2949            & 105          & 52.28 & 55.48 & 11.26 & 13.64 & 10.68 & 10.50 & 10.54 & 8.60  & 14.51 & 13.82 \\
CH4       & 18        & 6892            & 163          & 71.14 & 59.24 & 17.58 & 13.58 & 13.89 & 9.54  & 8.60  & 11.04 & 16.74 & 16.06 \\
B2        & 20        & 2239            & 64           & 84.96 & 72.70 & 23.94 & 20.23 & 16.00 & 13.06 & 6.31  & 7.42  & 16.64 & 16.26 \\
O2        & 20        & 2239            & 67           & 85.89 & 72.84 & 24.57 & 20.16 & 15.55 & 12.95 & 7.46  & 9.04  & 16.43 & 16.18 \\
Be2       & 20        & 2951            & 74           & 89.56 & 78.67 & 24.98 & 22.16 & 16.10 & 14.06 & 7.42  & 8.40  & 17.13 & 16.95 \\
C2        & 20        & 2951            & 75           & 90.34 & 78.06 & 25.36 & 21.83 & 15.97 & 13.55 & 7.23  & 8.51  & 17.28 & 17.24 \\
F2        & 20        & 2951            & 76           & 88.66 & 77.15 & 25.09 & 22.06 & 16.57 & 13.95 & 7.36  & 8.32  & 16.86 & 16.42 \\
Li2       & 20        & 2951            & 78           & 90.81 & 77.22 & 25.87 & 21.96 & 17.04 & 13.67 & 7.12  & 8.40  & 16.87 & 16.58 \\
N2        & 20        & 2951            & 79           & 93.53 & 79.00 & 27.10 & 22.10 & 16.90 & 13.91 & 6.86  & 8.41  & 17.35 & 17.06 \\ \bottomrule
\end{tabular}%
}
\end{table*}

==> src/Tables/n_meas_bk.tex <==
\begin{table*}[]
\centering
\caption{Statistics for the measurement circuits for each molecule's Bravyi-Kitaev mapping.}
\label{tab:n_meas_bk}
\begin{tabular}{@{}ccccccccc@{}}
\toprule
\textbf{Molecule} &
  \textbf{\# Qubits} &
  \textbf{\# Measurements} &
  \textbf{\# Groupings} &
  \textbf{Avg total gates} &
  \textbf{Avg 2Q gates} &
  \textbf{Avg Depth} &
  \textbf{Avg $r_{2q}$} &
  \textbf{Avg $k$} \\ \midrule
H$_2$   & 4  & 15   & 2   & 5.00  & 0.00  & 1.50  & - & 4.00  \\
HF      & 12 & 631  & 38  & 41.61 & 9.79  & 10.53 & 6.53     & 10.26 \\
LiH     & 12 & 631  & 41  & 38.07 & 8.27  & 9.41  & 7.76     & 10.46 \\
BeH$_2$ & 14 & 666  & 36  & 47.33 & 11.47 & 11.17 & 7.53     & 11.31 \\
H$_2$O  & 14 & 1086 & 50  & 48.98 & 11.52 & 10.76 & 7.65     & 11.98 \\
BH$_3$  & 16 & 1957 & 76  & 48.85 & 10.29 & 10.45 & 11.47    & 14.40 \\
NH$_3$  & 16 & 2949 & 105 & 52.28 & 11.26 & 10.68 & 10.54    & 14.51 \\
CH$_4$  & 18 & 6892 & 163 & 71.14 & 17.58 & 13.89 & 8.60     & 16.74 \\
B$_2$   & 20 & 2239 & 64  & 84.96 & 23.94 & 16.00 & 6.31     & 16.64 \\
O$_2$   & 20 & 2239 & 67  & 85.89 & 24.57 & 15.55 & 7.46     & 16.43 \\
Be$_2$  & 20 & 2951 & 74  & 89.56 & 24.98 & 16.10 & 7.42     & 17.13 \\
C$_2$   & 20 & 2951 & 75  & 90.34 & 25.36 & 15.97 & 7.23     & 17.28 \\
F$_2$   & 20 & 2951 & 76  & 88.66 & 25.09 & 16.57 & 7.36     & 16.86 \\
Li$_2$  & 20 & 2951 & 78  & 90.81 & 25.87 & 17.04 & 7.12     & 16.87 \\
N$_2$   & 20 & 2951 & 79  & 93.53 & 27.10 & 16.90 & 6.86     & 17.35 \\ \bottomrule
\end{tabular}
\end{table*}

==> src/Tables/n_meas_jw.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\centering
\caption{Statistics for the measurement circuits for each molecule's Jordan-Wigner mapping.}
\label{tab:n_meas_jw}
\begin{tabular}{@{}ccccccccc@{}}
\toprule
\textbf{Molecule} &
  \textbf{\# Qubits} &
  \textbf{\# Messurements} &
  \textbf{\# Groupings} &
  \textbf{Avg total gates} &
  \textbf{Avg 2Q gates} &
  \textbf{Avg Depth} &
  \textbf{Avg $r_{2q}$} &
  \textbf{Avg $k$} \\ \midrule
H$_2$   & 4  & 15   & 2   & 12.00 & 2.50  & 4.50  & 2.40  & 3.50  \\
HF      & 12 & 631  & 38  & 38.34 & 8.89  & 7.89  & 7.12  & 9.82  \\
LiH     & 12 & 631  & 41  & 36.34 & 8.34  & 8.15  & 7.24  & 9.54  \\
BeH$_2$ & 14 & 666  & 36  & 43.83 & 10.36 & 9.69  & 8.40  & 11.31 \\
H$_2$O  & 14 & 1086 & 50  & 46.88 & 11.46 & 9.78  & 7.58  & 11.36 \\
BH$_3$  & 16 & 1957 & 76  & 53.15 & 13.11 & 10.03 & 8.93  & 13.57 \\
NH$_3$  & 16 & 2949 & 105 & 55.48 & 13.64 & 10.50 & 8.60  & 13.82 \\
CH$_4$  & 18 & 6892 & 163 & 59.24 & 13.58 & 9.54  & 11.04 & 16.06 \\
B$_2$   & 20 & 2239 & 64  & 72.70 & 20.23 & 13.06 & 7.42  & 16.26 \\
O$_2$   & 20 & 2239 & 67  & 72.84 & 20.16 & 12.95 & 9.04  & 16.18 \\
Be$_2$  & 20 & 2951 & 74  & 78.67 & 22.16 & 14.06 & 8.40  & 16.95 \\
C$_2$   & 20 & 2951 & 75  & 78.06 & 21.83 & 13.55 & 8.51  & 17.24 \\
F$_2$   & 20 & 2951 & 76  & 77.15 & 22.06 & 13.95 & 8.32  & 16.42 \\
Li$_2$  & 20 & 2951 & 78  & 77.22 & 21.96 & 13.67 & 8.40  & 16.58 \\
N$_2$   & 20 & 2951 & 79  & 79.00 & 22.10 & 13.91 & 8.41  & 17.06 \\ \bottomrule
\end{tabular}
\end{table*}

==> src/background.tex <==
\subsection{Quantum Computing Background}

A quantum state on a single qubit is represented as $\ket{\psi} = \alpha\ket{0} + \beta\ket{1}$, a linear combination of basis states $\ket{0}$ and $\ket{1}$, where $\alpha$ and $\beta$ are complex coefficients that satisfy $|\alpha|^2 + |\beta|^2 = 1$. An $n$-qubit quantum state is similarly a linear combination of $2^n$ basis states $\ket{b_0 \ldots b_{n-1}}$.

Quantum gates are operations that act on qubits to transform one quantum state into another. The set of single-qubit gates and two-qubit controlled gates is universal, in that they can be combined to construct any quantum gate~\cite{nielsen2002quantum}. A quantum circuit is a series of quantum gates applied sequentially to transform the initial quantum state into the desired solution state.



==> src/structures/graph.tex <==

\begin{definition}
    A PoPR graph $G=(V,E)$ is a directed acyclic graph whose vertices $V$ are
    PoPR nodes (rotations, frames, preparations, and measurements),
    and whose edges $E \subseteq V \times V$ are antireflexive and
    asymmetric, and satisfy
    \begin{align*}
        \forall v_1, v_2 \in V,~ \commute*{v_1}{v_2}
            \iff (v_1,v_2) \in E
            \xor
            (v_2,v_1) \in E
    \end{align*}
\end{definition}
In other words, for any two vertices $n_1$ and $n_2$ that do not commute, there
is either an edge from $n_1$ to $n_2$ or vice versa (but not both). There are no
edges between commuting vertices.

% Note that for any topological sort $v_0,\ldots,v_{m-1}$, there is
% a unique way to add a new vertex $v$ at index $i$; any non-commutative nodes
% $v_0,\ldots,v_{i-1}$ will be given an edge into $v$, and any non-commutative 
% nodes $v_{i},\ldots,v_{m-1}$ will be given an edge out of $v$.

%\subsection{Semantics of a PoPR graph}
%\label{sec:PoPR-graph-semantics}

Every topological ordering of a PoPR graph $G$ corresponds to a PoPR term. Note
that even though topological orderings of a graph are not unique, all
corresponding PoPR terms will be equivalent to each other due to
\cref{thm:PoPRNodeCommuteCorrect}: if two vertices do not commute, there is an
edge between them in one direction or the other, and that edge will always be
preserved by the topological ordering.

\begin{ExtendedVersion}
\begin{lemma}
    For any two topological orderings $(v_0,\ldots,v_{m-1})$ and
    $(v_0',\ldots,v_{m-1}')$ of the same graph $G$,
    \begin{align*}
        v_0; \cdots; v_{m-1}
        \equiv
        v_0'; \cdots; v_{m-1}'.
    \end{align*}
\end{lemma}
\end{ExtendedVersion}


\begin{definition}
    Let $G$ be a PoPR graph and let $(v_0,\ldots,v_{m-1})$ be any topological
    ordering of its vertices. Then the semantics of $G$ as a Pauli map is given by
    \begin{align*}
        \interpM{G} &= \interpM{v_0;\cdots;v_{m-1}}
            = \interpM{v_{m-1}} \circ \cdots \circ \interpM{v_0}.
    \end{align*}
\end{definition}


\begin{ExtendedVersion}
Similarly, any PoPR term $t$ can be converted into a PoPR graph $G^t$.
First, $t$ can be written as an equivalent \emph{linear} PoPR term 
of the form $v_0;\ldots;v_{n-1}$ by associativity and identity rules.
Then the graph $G^t$ has vertices $\{v_0,\ldots,v_{n-1}\}$ and has an edge
$(v_i,v_j)$ if and only if both $\commute*{v_i}{v_j}$ and $i < j$.

\begin{lemma}
    For any PoPR term $t$ and Pauli $Q$,
    \begin{align*}
        \interpM{G^t}(Q) &\equiv \interpM{t}(Q).
    \end{align*}
\end{lemma}

Under this semantics, a PoPR graph essentially describes an equivalence class of PoPR terms.
Transformations on PoPR graphs can then be thought of as transformations on
PoPR terms: (1) convert a PoPR graph into a linear PoPR term corresponding to a
topological ordering of its vertices; (2) apply the transformation on the PoPR
term; and (3) convert the PoPR term back into a PoPR graph.

Going into further detail, to apply a particular optimization like $n_1;n_2 \rightarrow t$
where $n_1$ and $n_2$ correspond to vertices in the PoPR graph, we first need to
find a topological ordering whereby $n_1$ and $n_2$ are next to each other. This is possible
exactly when either (1) $n_1$ and $n_2$ commute and have exact same set of edges; or
(2) $n_1$ and $n_2$ do not commute and have distance $1$.
\end{ExtendedVersion}

PoPR graphs will always satisfy two additional invariants, explained in the rest of this section.
\begin{enumerate}
    \item \emph{Frame-terminal:} A well-formed PoPR graph contains a single Pauli frame node, which always occurs at the very end of the circuit; and
    \item \emph{Fully merged:} A well-formed PoPR graph contains no mergeable nodes.
\end{enumerate}

\subsubsection{Frame-terminal graphs}

A PoPR graph is called \emph{frame-terminal} when it contains a single Pauli frame node, which always occurs at the very end of the circuit. It is always possible to construct a frame-terminal graph because Pauli frames can always be commuted past other terms by mapping them onto their Pauli arguments. For a Pauli frame $F$ and a PoPR node $n$, we define $F(n)$ to be a new node $n'$ such that $n' \equiv n;F$.
\begin{align*}
    F(n) &= \begin{cases}
        F \circ F' & n=F' \\
        \Rot{F(P)}{\theta} & n = \Rot{P}{\theta} \\
        \Prep{F(P_Z)}{F(P_X)} & n=\Prep{P_Z}{P_X} \\
        \Meas[c]{F(P)} & n=\Meas[c]{P}
    \end{cases}
\end{align*}

\begin{lemma}
    $F; n \equiv F^{-1}(n); F$.
\end{lemma}

\subsubsection{Mergeable nodes}

A pair of nodes $(n_1,n_2)$ is called \emph{mergeable} if they occur next to each other in the graph (the longest path between them has length 1) and there is a step $n_1;n_2 \mergestep t$ to a new Pauli term, as shown in \cref{fig:MergeVerticesStep}. For such a merge to occur, $n_1$ and $n_2$ must have the same underlying Pauli arguments, modulo $\pm 1$, in which case they can be combined into a single node, or in the case of measurement, two new but still simpler nodes. 

\begin{figure*}
    \centering
\begin{align*}\begin{array}{c}
    \inferrule*
        { \theta = \theta_1 \pm \theta_2~\text{is a multiple of}~\tfrac{\pi}{2}
        }
        { \Rot{P}{\theta_1}; \Rot{\pm P}{\theta_2}
            \mergestep
            \frameof{P, \theta}
        }
    \\ \\
    \inferrule*
        { \theta = \theta_1 \pm \theta_2~\text{not a multiple of}~\tfrac{\pi}{2}
        }
        { \Rot{P}{\theta_1}; \Rot{\pm P}{\theta_2}
            \mergestep
            \Rot{P}{\theta}
        }
\end{array} \end{align*}
\begin{align*}
    \Prep{P_Z}{P_X}; \Prep{\pm P_Z}{P_X'}
            &\mergestep
            \Prep{\pm P_Z}{P_X'} \\
    \Rot{P_Z}{\theta}; \Prep{\pm P_Z}{P_X}
            &\mergestep
            \Prep{\pm P_Z}{P_X} \\
    \Meas[c_1]{P}; \Meas[c_2]{\pm P}
            &\mergestep
            \Meas[c_1 ++ c_2]{\pm P} \\
    \Prep{P_Z}{P_X}; \Meas[c]{\pm P_Z}
            &\mergestep
            \Prep{P}{P_X}; \Meas[c]{\pm I} \\
    \Rot{\pm P}{\theta}; \Meas[c]{P}
            &\mergestep
            \Meas[c]{P}
\end{align*}
\begin{align*}
    \merge{n_1}{n_2} &= \begin{cases}\begin{aligned}
        &\frameof{P, \theta}
            \qquad \qquad
            &&  n_1 = \Rot{P}{\theta_1} 
            \wedge
                n_2=\Rot{\pm P}{\theta_2}
            &\wedge~& 
                \theta = \theta_1 \pm \theta_2 ~\text{a multiple of}~\tfrac{\pi}{2}
                \\
        &\Rot{P}{\theta}
            &&  n_1 = \Rot{P}{\theta_1}
            \wedge
                n_2=\Rot{\pm P}{\theta_2}
            &\wedge~&
                \theta = \theta_1 \pm \theta_2 ~\text{not a multiple of}~\tfrac{\pi}{2}
                \\
        &\Prep{P_Z'}{P_X'}
            &&  n_1 = \Prep{P_Z}{P_X}
            \wedge
                n_2 = \Prep{P_Z'}{P_X'}
            &\wedge~&
                P_Z' = \pm P_X'
                \\
        &\Prep{P_Z}{P_X}
            &&  n_1 = \Rot{P}{\theta}
            \wedge
                n_2 = \Prep{P_Z}{P_X}
            &\wedge~&
                P_Z = \pm P
        \\
        &\Meas[c_1 ++ c_2]{\pm P}]
            && n_1 = \Meas[c_1]{P}
            \wedge
                n_2 = \Meas[c_2]{P}
        \\
        &\Prep{P_Z}{P_X}; \Meas[c]{\pm I}
            &&  n_1 = \Prep{P_Z}{P_X}
            \wedge
                n_2 = \Meas[c]{P_Z'}
            &\wedge~&
                P_Z' = \pm{P_Z}
        \\
        &\Meas[c]{P'}
            &&  n_1 = \Rot{P}{\theta}
            \wedge
                n_2 = \Meas[c]{P'}
            &\wedge~& P' = \pm P
        \\
        &\text{undefined}
            &&\text{otherwise}
    \end{aligned} \end{cases}
\end{align*}
    \caption{Rules for merging vertices. \jennifer{Which version looks better?} When $\theta$ is a multiple of $\frac{\pi}{2}$, it will be the case that $\Rot{P}{\theta}$ is a Clifford unitary, and we refer to the corresponding Pauli frame as $\frameof{P,\theta}$, as in \cref{fig:CliffordFrame}.
    }
    \label{fig:MergeVerticesStep}
\end{figure*}

\begin{lemma}
    If $t_1 \mergestep t_2$
    then $t_1 \equiv t_2$.
\end{lemma}
\begin{ExtendedVersion}
    \todo{proof--uses the rules from \cref{sec:PoPR}.}
\end{ExtendedVersion}


==> src/structures/popr.tex <==

A \emph{PoPR node} $n$ is
one of these four structures, and a \emph{PoPR term} $t$ is the monoidal
composition of PoPR nodes with the identity as a unit.
\begin{align*}
    n &::= \Rot{P}{\theta}  \mid F \mid \Meas[c]{P} \mid \Prep{P_1}{P_2} \\
    t &::= 1 \mid n \mid t_1; t_2
\end{align*}

The semantics of PoPR terms is given as Pauli maps. Note that while 
unitary terms (Pauli rotations and frames) are 
given semantics as Pauli vectors $\interp{n}$, those vectors
can be lifted to Pauli maps by conjugation:
\begin{align*}
    \interpM{n}(Q) &= \conjugate{\interp{n}}{Q} = \interp{n}^\dagger Q \interp{n}
        &n~\text{unitary}\\
    %\interpM{\alpha}(Q) &= |\alpha| Q \\
    \interpM{1}(Q) &= Q \\
    \interpM{t_1; t_2}(Q) &= \interpM{t_2}(\interpM{t_1}(Q))
\end{align*}

\albert{What does the M stand for?} 
\jennifer{It's just syntax to distinguish it from $\interp{v}$; maybe find a
better syntax.}

\begin{ExtendedVersion}
Note that since the action of the PoPR nodes' semantics as Pauli maps
is linear on their Paulis, when we lift the Pauli map $\interpM{n}$ to operate on
vectors, it is equivalent to substitute $n$ for $P$ in the definition.\footnote{This applies to all PoPR nodes except Pauli frames.}
\begin{lemma} \label{lem:PauliNodeSubstitution}
    \begin{align*}
        &\interpM{\Rot{P}{\theta}}(v) 
            = \interp{\Rot{P}{-\theta}} v \interp{\Rot{P}{\theta}} \\
        &\interpM{\Prep{P_Z}{P_X}}(v) \\
            &= (I + P_Z) v (I + P_Z) + P_X (I - P_Z) v (I - P_Z) P_X \\
        &\interpM{\Meas[c]{P}}(v) \\
            &= (I + P) v (I + P) + (I - P) v (I - P)
    \end{align*}
\end{lemma}
\end{ExtendedVersion}


We can define an equivalence relation on the PoPR monoid based on this semantics:
\begin{align*}
    t_1 \equiv t_2 
    \iff
    \forall Q,~ \interpM{t_1}(Q) = \interpM{t_2}(Q)
\end{align*}

\begin{ExtendedVersion}
First, we establish that sequential composition $t_1; t_2$ forms a monoid with
$1$ as the unit.
\begin{lemma}
    \begin{align*}
        1; t &\equiv t;1 \equiv t \\
        (t_1 ; t_2); t_3 &\equiv t_1 ; (t_2 ; t_3)
    \end{align*}
\end{lemma}
\end{ExtendedVersion}


\begin{comment}
\begin{figure}
    \centering
  \begin{align}
    \Rot{P}{\theta_1}; \Rot{P}{\theta_2} &\equiv \Rot{P}{\theta_1 + \theta_2} \\
    \Rot{P}{0} &\equiv 1 \\
    \Rot{P}{\theta}^\dagger &\equiv \Rot{P}{-\theta} \\
    \Rot{P}{\pi} &\equiv \pauliToFrame{P} \\
    \Rot{P}{\frac{\pi}{2}} &\equiv \pauliToFrame2{P}
  \end{align}
    \caption{Properties of single-axis rotations.}
    \label{fig:RotEquivProperties}
\end{figure}

\begin{comment}
\begin{figure}
    \centering
    \begin{align}
        \Meas[c_1]{P}; \Meas[c_2]{P}
            &\equiv
            \Meas[c_1 \plusplus c_2]{P}
            \\
        \Meas[c]{-P}
            &\equiv
            \Meas[c]{P}
            \\
        \Prep{P_Z}{P_X}; \Prep{P_Z}{P_X'}
            &\equiv
            \Prep{P_Z}{P_X}
            \\
        \Prep{P_Z}{P_X}
            &\equiv
            \Prep{P_Z}{-i P_Z P_X}
            \\
        \Prep{P_Z}{P_X}
            &\equiv
            \Prep{P_Z}{-P_X}
            \\
        \Rot{P_Z}{\theta}; \Prep{P_Z}{P_X}
            &\equiv
            \Prep{P_Z}{P_X}
            \\
        \Prep{P_Z}{P_X}; \Rot{P_Z}{\theta}
            &\equiv
            \Prep{P_Z}{P_X}
            \label{eqn:RotPrepEquiv}
            \\
        \Rot{P}{\theta}; \Meas[c]{P}
            &\equiv
            \Meas[c]{P}
            \label{eqn:RotMeasEquiv}
            \\
        \Prep{P_Z}{P_X}; \Meas[c]{P_Z}
            &\equiv
            \Prep{P_Z}{P_X}; \Meas[c]{I}
    \end{align}
    \caption{Properties of measurement and preparations.
    \jennifer{We may also want to give a semantics to the classical channels appearing
in measurements, otherwise the last equation it's silly to have the final measurement.}
    \albert{May need an extra swap gate on the measurement, e.g. $c \Rightarrow \neg c$}
    }
    \label{fig:MeasPrepEquivProperties}
\end{figure}
\end{comment}


\begin{ExtendedVersion}
\begin{proof}[Proof of \cref{eqn:RotPrepEquiv}]
\begin{align*}
    &  \left(\interpM{\Prep{P_Z}{P_X}}; \interpM{\Rot{P_Z}{\theta}}\right)(Q) \\
    &= \interpM{\Rot{P_Z}{\theta}}(\interpM{\Prep{P_Z}{P_X}}(Q)) \\
    &= \interpM{\Rot{P_Z}{\theta}}\left(
        \begin{cases}
            Q (I + P_Z) & \commutativity{Q}{P_Z}=\commutativity{Q}{P_X}=0 \\
            0 & \text{otherwise}
        \end{cases}\right) \\
    &= \begin{cases}
          \interp{\Rot{P_Z}{-\theta}} Q (I + P_Z) \interp{\Rot{P_Z}{\theta}}
            & \parbox[t]{1cm}{\ensuremath{
                \commutativity{Q}{P_Z}=\commutativity{Q}{P_X}=0
            }} \\
          0 & \text{otherwise}
        \end{cases}
\end{align*}
In the case when $\commute{Q}{P_Z}$ and $\commute{Q}{P_X}$ it is easy to check that
$\interp{\Rot{P_Z}{-\theta}} Q (I + P_Z) = Q (I + P_Z) \interpM{\Rot{P_Z}{\theta}}$, in which case
\begin{align*}
    &\interp{\Rot{P_Z}{-\theta}} Q (I + P_Z) \interp{\Rot{P_Z}{\theta}} \\
    &= Q (I + P_Z) \interp{\Rot{P_Z}{-\theta}} \interp{\Rot{P_Z}{\theta}} \\
    &= Q (I + P_Z) I
\end{align*}
and is thus equal to $\interpM{\Prep{P_Z}{P_X}}(Q)$.
\end{proof}
\end{ExtendedVersion}

\begin{figure}
    \centering
\begin{align} 
    F_1 ; F_2 &\equiv (F_2 \circ F_1) \\ 
    F^0 &\equiv 1 \\
    F ; \Rot{P}{\theta}
        &\equiv
        \Rot{F^{-1}(P)}{\theta}; F \\
    F ; \Meas[c]{P}
        &\equiv
        \Meas[c]{F^{-1}(P)}; F \\
    F ; \Prep{P_1}{P_2}
        &\equiv
        \Prep{F^{-1}(P_1)}{F^{-1}(P_2)}
\end{align}
    \caption{Properties of Pauli frames}
    \label{fig:FrameEquivProperties}
\end{figure}


Intuitively, two PoPR nodes commute exactly when their underlying
Paulis commute. To show this, we define a new syntactic
relation $\commute{n}{n'}$ (\cref{fig:CommuteTermTerm}) and prove  in \cref{thm:PoPRNodeCommuteCorrect} that $\commute{n}{n'}$ implies
$\interpM{n; n'} \equiv \interpM{n'; n}$.
This relation is aided by two helper relations
$\commute{P}{n}$ (\cref{fig:CommutePauliNode}, indicating when a Pauli commutes with a PoPR node) and
$\commute{F}{F}$ (when two Pauli frames commute)\footnotemark,
which holds exactly when $F \circ F' = F' \circ F$.

\footnotetext{
These definitions are given as inference rules, a standard
presentation in formal logic. The way to read such an inference rule is as
follows: the relation below the line (the conclusion) holds if and only if all
the relations above the line (the hypotheses) hold.}


\begin{figure}
\begin{align*} \begin{array}{c}
    \inferrule*[right=Rot-\commuteTPRule]
        {\commute{Q}{P}}
        {\commute{Q}{\Rot{P}{\theta}}}
    \qquad
    \inferrule*[right=F-\commuteTPRule]
        {F(Q)=Q}
        {\commute{Q}{F}}
    \\ \\
    \inferrule*[right=Prep-\commuteTPRule]
        {\commute{Q}{P_1} \\ \commute{Q}{P_2}}
        {\commute{Q}{\Prep{P_1}{P_2}}}
    \quad
    \inferrule*[right=Meas-\commuteTPRule]
        {\commute{Q}{P}}
        {\commute{Q}{\Meas[c]{P}}}
    % \qquad
    % \inferrule*[right=const-\commuteTPRule]
    %     {~}
    % %     {\commute{Q}{\alpha}}
    % \qquad
    % \inferrule*[right=seq-\commuteTPRule]
    %     {\commute{Q}{t_1} \\ \commute{Q}{t_2}}
    %     {\commute{Q}{t_1; t_2}}
    % \\ \\
\end{array} \end{align*}
\caption{Definition of $\commute{P}{n}$. Recall that for two Paulis, we write $\commute{P_1}{P_2}$ if and only if
$\commutativity{P_1}{P_2} = 0$.}
\label{fig:CommutePauliNode}
\end{figure}

\begin{figure}
\begin{align*} \begin{array}{c}
    \inferrule*[right=Rot-\commuteTTRule]
        {\commute{P}{n}}
        {\commute{\Rot{P}{\theta}}{n}}
    \\ \\
    \inferrule*[right=F-\commuteTTRule]
        {n~\text{not a Pauli frame} \\ \commute{n}{F}}
        {\commute{F}{n}}
    \\ \\
    \inferrule*[right=Prep-\commuteTTRule]
        {\commute{P_1}{n} \\ \commute{P_2}{n}}
        {\commute{\Prep{P_1}{P_2}}{n}}
    \quad
    \inferrule*[right=Meas-\commuteTTRule]
        {\commute{P}{n}}
        {\commute{\Meas[c]{P}}{n}}
\end{array} \end{align*}
\caption{Definition of $\commute{n_1}{n_2}$ indicating when two PoPR nodes commute.}
\label{fig:CommuteTermTerm}
\end{figure}


\begin{lemma} \label{lem:CommuteTPCorrect}
    If $\commute{Q}{n}$ then
    \begin{align*}
        \interpM{n}(Q) = \begin{cases}
            Q (I + P_Z) & n = \Prep{P_Z}{P_X} \\
            Q & \text{otherwise}
        \end{cases}
    \end{align*}
\end{lemma}
\begin{ExtendedVersion}
\begin{proof}
By induction on the derivation of $\commute{Q}{n}$.
    \proofpart[$n = \Rot{P}{\theta}$]
    Assume $\commute{P}{Q}$; to show
    $\interpM{\Rot{P}{\theta}}(Q)=Q$, it suffices
    to show that $Q$ commutes with $\interp{\Rot{P}{\theta}}$:
    \begin{align*}
        \interp{\Rot{P}{\theta}} \cdot Q
            &= (\cos{\tfrac{\theta}2} I - i \sin{\tfrac{\theta}2} P) Q \\
            &= \cos{\tfrac{\theta}2} Q - i \sin{\tfrac{\theta}2} P Q \\
            &= \cos{\tfrac{\theta}2} Q - i \sin{\tfrac{\theta}2} Q P 
                \tag{$\commute{P}{Q}$} \\
            &= Q (\cos{\tfrac{\theta}2} I - i \sin{\tfrac{\theta}2} P)
            = Q \cdot \interp{\Rot{P}{\theta}}
    \end{align*}
    
    \proofpart[$n = F$]
    Follows by definition.

    \proofpart[$n = \Prep{P_Z}{P_X}$]
    Assume $\commute{P_Z}{Q}$ and $\commute{P_X}{Q}$. Then
    \begin{align*}
        &\interpM{\Prep{P_Z}{P_X}}(Q) \\
        &= \frac{1}{4} \left( (I + P_Z)Q(I+P_Z) + P_X(I - P_Z)Q(I-P_Z)P_X \right) \\
        &= \frac{1}{4} \left(
                Q (I + P_Z)(I + P_Z) + Q P_X (I-P_Z)(I-P_Z) P_X
            \right) 
            \tag{$\commute{Q}{P_Z}$ and $\commute{Q}{P_X}$} \\
        &=  \frac{1}{4} Q \left(
                2(I + P_Z) + P_X 2(I-P_Z) P_X
            \right) \\
        &=  \frac{1}{4} Q \left(
                2(I + P_Z) + 2(I+P_Z) P_X P_X
            \right) \\
        &= Q (I + P_Z) = (I + P_Z) Q
    \end{align*}

    \proofpart[\ensuremath{n = \Meas[c]{P}}]
    Assuming $\commute{P}{Q}$, we can see that
    \begin{align*}
        \interpM{\Meas[c]{P}}(Q)
        &= \frac{1}{4} \left( (I + P)Q(I + P) + (I - P)Q(I-P) \right) \\
        &= \frac14 Q \left(
                (I + P)(I + P) + (I - P)(I - P)
            \right)
            \tag{$\commute{Q}{P}$} \\
        &= \frac14 Q \left(
                2(I + P) + 2(I - P)
            \right)
        = Q \qedhere
    \end{align*}
\end{proof}
\end{ExtendedVersion}

\begin{ExtendedVersion}
A unitary node $n$ is either a rotation or Pauli frame, and unitary nodes
distribute over multiplication of Pauli vectors. Note that by
\cref{lem:MonoidalMapsNatural} and \cref{lem:FrameCompositionNatural}, unitary
nodes respect multiplication of Pauli vectors.
\end{ExtendedVersion}

\begin{theorem} \label{thm:PoPRNodeCommuteCorrect}
    If $\commute{n_1}{n_2}$ then $n_1; n_2 \equiv n_2; t_1$.\footnotemark
\end{theorem}
\footnotetext{Note that this property does not hold in the other direction; the rules for $\commute{n_1}{n_2}$ are strictly more
restrictive. In particular, the relation is not reflexive on $\Prep{P_Z}{P_X}$ since $\anticommute{P_Z}{P_X}$.
}
\begin{ExtendedVersion}
\begin{proof}
    By induction on the derivation of $\commute{n_1}{n_2}$.

    \proofpart[$n_1=\Prep{P_Z}{P_X}$ and $n_2=\Prep{P_Z'}{P_X'}$]
    Let $n_1=\Prep{P_Z}{P_X}$ such that
    $\commute{P_Z}{n_2}$ and $\commute{P_X}{n_2}$, and
    let $n_2$ be $\Prep{P_Z'}{P_X'}$, in which it
    will be the case that
    $P_Z$ and $P_X$ each commute with both $P_Z'$ and $P_X'$.
    Then
    \begin{align}
        &\interpM{n_2}(\interpM{n_1}(Q)) \notag \\
        &= \interpM{\Prep{P_Z'}{P_X'}}\left(
            \interpM{\Prep{P_Z}{P_X}}(Q)
        \right) \notag \\
        &= \interpM{\Prep{P_Z'}{P_X'}}\left(
            \begin{cases}
                Q(I + P_Z) & \commutativity{Q}{P_Z} = \commutativity{Q}{P_X} = 0 \\
                0          & \text{otherwise}
            \end{cases}
        \right) \notag \\
        &=  \begin{cases}
                \interpM{\Prep{P_Z'}{P_X'}}\left(Q(I + P_Z)\right)
                    & \commutativity{Q}{P_Z} = \commutativity{Q}{P_X} = 0 \\
                0   
                    & \text{otherwise}
            \end{cases} \notag \\
        &= \begin{cases}
                \interpM{\Prep{P_Z'}{P_X'}}(Q)\\
                ~+
                \interpM{\Prep{P_Z'}{P_X'}}(Q P_Z)
                    & \commutativity{Q}{P_Z} = \commutativity{Q}{P_X} = 0 \\
                0
                    & \text{otherwise}
            \end{cases} \label{eqn:PrepIntermediary}
    \end{align}
    In the case that $\commutativity{Q}{P_Z} = \commutativity{Q}{P_X} = 0$,
    we have that
    \begin{align*}
        &\interpM{\Prep{P_Z'}{P_X'}}(Q P_Z) \\
        &= \begin{cases}
            Q P_Z (I + P_Z')  & \commutativity{QP_Z}{P_Z'}= \commutativity{Q P_Z}{P_X'} = 0 \\
            0           & \text{otherwise}
        \end{cases}
    \end{align*}
    However, in that case
    \begin{align*}
        \commutativity{Q P_Z}{P_Z'}
        &= \commutativity{Q}{P_Z'} + \commutativity{P_Z}{P_Z'}
        = \commutativity{Q}{P_Z'}
    \end{align*}
    since $\commutativity{P_Z}{P_Z'} = 0$, and similarly
    $\commutativity{Q P_Z}{P_X'} = \commutativity{Q}{P_X'}$.
    Thus \cref{eqn:PrepIntermediary}
    becomes 
    \begin{align*}
        &\begin{cases}
            Q(I + P_Z') + Q P_Z (I + P_Z')
                & \commutativity{Q}{P_Z} = \commutativity{Q}{P_X} = 0 \\
                &\wedge \commutativity{Q}{P_Z'} = \commutativity{Q}{P_X'} = 0 \\
            0   & \text{otherwise}
        \end{cases} \\
        = &\begin{cases}
            Q(I + P_Z)(I + P_Z')
                & \commutativity{Q}{P_Z} = \commutativity{Q}{P_X} \\ 
                &= \commutativity{Q}{P_Z'} = \commutativity{Q}{P_X'} = 0 \\
            0   & \text{otherwise}
        \end{cases}
    \end{align*}

    Notice that all the above reasoning applies for
    $\interpM{n_1}(\interpM{n_2}(Q))$
    as well,
    which becomes
    \begin{align*}
        \begin{cases}
            Q(I + P_Z')(I + P_Z)
                & \commutativity{Q}{P_Z} = \commutativity{Q}{P_X} \\
                &= \commutativity{Q}{P_Z'} = \commutativity{Q}{P_X'} = 0 \\
            0   & \text{otherwise}
        \end{cases}
    \end{align*}
    Because $\commute{P_Z}{P_Z'}$, we must have $Q(I + P_Z)(I + P_Z') = Q (I + P_Z')(I + P_Z)$,
    and so these two results are equal.

    \proofpart[$n_1=\Prep{P_Z}{P_X}$ and $n_2=\Meas{P}$]

    Next assume $n_1=\Prep{P_Z}{P_X}$ and $n_2=\Meas{P}$, in which case
    $\commute{P_Z}{P}$ and $\commute{P_X}{P}$. Then 
    \begin{align*}
        &\interpM{n_1}\left(
            \interpM{n_2}(Q)
        \right) \\
        &= 
        \interpM{n_2}\left(
            \begin{cases}
                Q & \commutativity{Q}{P} = 0 \\
                0 & \text{otherwise}
            \end{cases}
        \right) \\
        &= 
        \begin{cases}
            \interpM{n_2}(Q) & \commutativity{Q}{P} = 0 \\
            0 & \text{otherwise}
        \end{cases} \\
        &= 
        \begin{cases}
            Q(I + P_Z) & \commutativity{Q}{P} = \commutativity{Q}{P_Z} = \commutativity{Q}{P_X} = 0 \\
            0 & \text{otherwise}
        \end{cases}
    \end{align*}

    On the other hand,
    \begin{align*}
        &\interpM{n_2}\left(
            \interpM{n_1}(Q)
        \right) \\
        &= 
        \interpM{n_2}\left(
            \begin{cases}
                Q(I + P_Z) & \commutativity{Q}{P_Z} = \commutativity{Q}{P_X} = 0 \\
                0 & \text{otherwise}
            \end{cases}
        \right) \\
        &= 
        \begin{cases}
            Q(I + P_Z) & \commutativity{Q}{P} = \commutativity{Q}{P_Z} = \commutativity{Q}{P_X} = 0 \\
            0 & \text{otherwise}
        \end{cases}
    \end{align*}
    which concludes the proof.

    \proofpart[$n_1=\Prep{P_Z}{P_X}$ and $n_2$ is unitary]

    \begin{align*}
        \interpM{n_2}(\interpM{n_1}(Q))
        = \frac14 \interpM{n_2} (
            &(I + P_Z) Q (I + P_Z) \\
            &+
            P_X (I - P_Z) Q (I - P_Z) P_X
        )
    \end{align*}
    Since $n_2$ is not a preparation, we know that 
    $\interpM{n_2}(P_X) = P_X$ and 
    $\interpM{n_2}(I \pm P_Z) = I \pm P_Z$;
    furthermore, since $n_2$ is unitary, it distributes over
    vector multiplication (\cref{lem:MonoidalMapsNatural});
    thus the equation above becomes
    \begin{align*}
        \frac14 (
            &(I + P_Z) \interpM{n_2}(Q) (I + P_Z) \\
            &+
            P_X (I - P_Z) \interpM{n_2}(Q) (I - P_Z) P_X
        ) \\
        &= \interpM{n_1}(\interpM{n_2}(Q))
    \end{align*}

    \proofpart[$n_1=\Meas{P}$ and $n_2=\Meas{P'}$]

    \begin{align*}
        &\interpM{\Meas{P}}\left(\interpM{\Meas{P'}}(Q)\right) \\
        &= \interpM{\Meas{P}}\left(
            \begin{cases}
                Q & \commute{P'}{Q} \\
                0 & \text{otherwise}
            \end{cases}
        \right) \\
        &= \begin{cases}
                Q & \commute{P'}{Q} \wedge \commute{P}{Q} \\
                0 & \text{otherwise}
            \end{cases} \\
        &= \interpM{\Meas{P'}}\left(\interpM{\Meas{P}}(Q)\right)
    \end{align*}

    \proofpart[$n_1=\Meas{P}$ and $n_2$ unitary]

    \begin{align*}
        &\interpM{n_2}(\interpM{n_1}(Q)) \\
        &= \interpM{n_2}\left(
            (I + Z) Q (I + Z) + (I - Z) Q (I - Z)
        \right)
    \end{align*}
    Similar to the case where $n_1$ is a preparation, since $n_2$ is \emph{not} a preparation
    we know that $\interpM{n_2}(I \pm Z) = I \pm Z$, and since it is unitary,
    it can distribute over vector multiplication (\cref{lem:MonoidalMapsNatural}),
    so this is equal to
    \begin{align*}
        &(I + Z) \interpM{n_2}(Q) (I + Z)
        + (I - Z) \interpM{n_2}(Q) (I - Z) \\
        &= \interpM{n_1}(\interpM{n_2}(Q))
    \end{align*}

    \proofpart[$n_1=\Rot{P}{\theta}$ and $n_2$ unitary]

    Assuming $\commute{n_2}{P}$, it must be the case that
    \begin{align*}
        \interpM{n_2}(\interp{\Rot{P}{\theta}})
        &= \interpM{n_2}\left(
            \cosBy2{\theta} I + i \sinBy2{\theta} P
        \right) \\
        &= \cosBy2{\theta} I + i \sinBy2{\theta} P = \interp{\Rot{P}{\theta}}
    \end{align*}
    Thus
    \begin{align*}
        &\interpM{n_2}(\interpM{\Rot{P}{\theta}}(Q)) \\
        &= \interpM{n_2}(\interp{\Rot{P}{-\theta}} Q \interp{\Rot{P}{\theta}}) \\
        &= \interpM{n_2}(\interp{\Rot{P}{-\theta}}) (\interpM{n_2}(Q)) \interpM{n_2}(\interp{\Rot{P}{\theta}})
            \tag{\cref{lem:MonoidalMapsNatural}} \\
        &= \interp{\Rot{P}{-\theta}} (\interpM{n_2}(Q)) \interp{\Rot{P}{\theta}} \\
        &= \interpM{\Rot{P}{\theta}}(\interpM{n_2}(Q))
    \end{align*}
     as desired.

\end{proof}
\end{ExtendedVersion}


==> src/structures/structures.tex <==
The Product-of-Pauli-Rotation (PoPR) optimization uses Pauli rotations to represent non-Clifford unitaries.

\begin{definition}
A Pauli rotation is a tuple $\Rot{P}{\theta}$ of a Hermitian Pauli $P$ on $n$
qubits and a real number $\theta \in \mathbb{R}$. The semantics of a Pauli
rotation is
  \begin{align*}
    \interp{\Rot{P}{\theta}} &= e^{-i \theta / 2 \interp{P}} \\
    &= \cos(\tfrac{\theta}{2}) I + i \sin(\tfrac{\theta}{2}) \interp{P}
  \end{align*}
\end{definition}

\citet{Zhang2019} define an optimization technique that commutes Cliffords past rotations of the form $\Rot{P}{\tfrac{\pi}{2}}$, since they were primarily concerned with the Clifford + T gateset. In this work we are focused on NISQ architectures, many of which support arbitrary single-qubit rotations. \todo{Move this discussion to introduction?} In addition, PoPR optimizations support not just unitaries, but also preparations and measurements. Generalizing these components by their Pauli axis as well, we can use the same technique to describe how Cliffords commute past them.

Ultimately, our PoPR optimizations will rely on four different types of nodes:
\begin{itemize}
    \item Pauli frames, representing Cliffords
    \item Pauli rotations, representing non-Clifford unitaries
    \item Pauli measurements
    \item Pauli preparations
\end{itemize}


\begin{definition}
    A Pauli measurement $\Meas[c]{P}$ 
    consists of a Hermitian Pauli representing the measurement operator.
    \begin{align*}
        &\interpM{\Meas[c]{P}}(Q) \\
        &=
        \frac{1}{4} \left( (I + P)Q(I + P) + (I - P)Q(I-P) \right) \\
        &=\begin{cases}
            Q & \commutativity{P}{Q}=0 \\
            0 & \text{otherwise}
        \end{cases}
    \end{align*}
\end{definition}

As an example, measuring qubit $i$ in the $Z$ basis would be represented as $\Meas[c]{Z_i}$.

The $c$ argument corresponds to the classical register(s) in which the measurement is being
recorded. We write $c \plusplus c'$ for the $n$-tuple with $(c \plusplus c')[i]=c[i] \plusplus c'[i]$.
Note that these registers are not relevant to the semantics, but are important when
converting back and forth between PoPR representations and circuits.

\jennifer{I think we really need to incorporate the registers into the semantics... TODO}


\begin{definition}
    A Pauli preparation
    $\Prep{P_1}{P_2}$ consists of a pair of non-commutative Hermitian Paulis where the first
    corresponds to the measurement basis and the second corresponds to the
    control operator.
    \begin{align*}        
        &\interpM{\Prep{P_Z}{P_X}}(Q) \\
        &=
        \frac{1}{4} \left( (I + P_Z)Q(I + P_Z) + P_X(I - P_Z)Q(I-P_Z)P_X \right) \\
        &= \begin{cases}
            Q (I + P_Z) & \commutativity{Q}{P_Z} = \commutativity{Q}{P_X} = 0 \\
            0           & \text{otherwise}
        \end{cases}
    \end{align*}
    %where $\conjugate{v}(Q) = v^\dagger Q v$ corresponds to conjugation by
    %a unitary $v$. \albert{I don't think you want to define this for only unitaries}
\end{definition}

For example, preparing the $i$th qubit in the $Z$ basis would be encoded as 
$\Prep{Z_i}{X_i}$.

==> src/synthesis.tex <==
After optimization of the PoPR graph, the next step is to synthesize a circuit with the equivalent channel action on any state. The methods closely follow those outlined in Ref. \cite{Schmitz2021} which we summarize here along with the modifications needed to accommodate the additional features of the PoPR graph.

We will always consider the synthesis of a frame-terminating, fully merged PoPR graph. Much the same way the PoPR graph is produced, we imagine prepending the PoPR graph with an empty circuit, then either moving those nodes free of dependency and which are directly supported by gate action into the circuit, or selecting a Clifford gate, and generating an identity on the overall logic whereby we add the gate to the circuit and transform the graph by the Clifford's inverse action (what we refer to as ``pushing to the circuit'' and ``pushing the the graph,'' respectively). Thus synthesis is primarily a method for selecting the sequence of Clifford gates which will minimize the gate cost, depth or some other cost metric of the resulting circuit. In particular, we consider choosing amongst the two-qubit entangling (TQE) gates as outlined in Ref. \cite{Schmitz2021} \albert{add visual of TQE gates?}. Likewise, we adapt the  heuristic ultra-greedy search algorithm with some abstractions which we refer to as the \emph{search functions}, of which there are four for a given type of search:
\begin{enumerate}
    \item NodeCost(n) - returns a cost to implement the node n (independent of $G$) with the promise that the cost is zero if and only if the node can be pushed to the circuit.
    \item ReduceNode(n) - returns a set of available TQE gates which reduces the NodeCost return value when the node n is conjugated by the gate. It also promises "monotonicity" with respects to NodeCost, i.e. for every gate it returns for a given node, that gate reduces NodeCost when the node is transformed by the gate, and the repeated process of apply any sequence of gates returned by the function will eventually reduce NodeCost to zero.
    \item GateCost($C:G$, $g$) - returns a cost value for the result of transforming $C$ and $G$ by the passed TQE gate but does not actually transform $C$ or $G$. It makes no additional promises.
    \item addGate(graph $C:G$, $g$) - Performs a logical identity across the boundary between $C$ and $G$, where by $g$ (or an appropriate equivalent) is add to $C$.
\end{enumerate}

Given these functions, we start with synthesizing the non-Clifford nodes. Let $\text{BEGIN}(G)$ be the set of all non-Clifford nodes free of dependency in the PoPR graph $G$. The ultra-greedy search algorithm is then as follows:

\begin{algorithm}
\caption{Ultra Greedy Search Algorithm Non-Clifford(G). \\
    Returns circuit and PoPR graph $C:G'$ such that $\termof{C:G'} \equiv \termof{G}$ and $G'$ is Clifford}
Let $G'$ be a copy of $G$ and prepend to it an empty circuit $C$.
While $G'$ contains non-Clifford nodes, do:
\begin{enumerate}
    \item For each $n \in \text{BEGIN}(G')$, if NodeCost(n) = 0, then apply addGate($C:G'$, $g(n)$); remove $n$ from $G'$.
    \item Compute MIN as the set of remaining terms in $\text{BEGIN}(G')$ which minimize NodeCost.
    \item Compute MINGate as the set ReduceNode(MIN).
    \item Compute a gate $g_{min}$ which minimizes GateCost($G':C$, MINGate) 
    \item apply addGate($C:G'$, $g_{min}$).
\end{enumerate}
Return $C:G'$
\label{algo:greedy}
\end{algorithm}

As argued in Ref. \cite{Schmitz2021}, this algorithm always terminates, primarily due to the promises made by the search functions. It should also be clear that $\termof{C:G'} \equiv \termof{G}$, as addGate always preforms a logical identity between the graph and the circuit.

\subsubsection{Implementations of the Search functions}
One can imagine several implementations of the search functions with varying complexities and cost considerations. Here, we discuss those currently implemented in the Intel Quantum SDK and some extension we shall consider in future work.
The most basic search functions use the number of TQE gates required to reduce the node cost to zero as the primary consideration. Calculation of NodeCost is then dependent on the type of the node as sorted into two categories: singlet nodes, and factor nodes. 

Singlet nodes are those defined by a single Pauli operator such as $\Rot$ and $\Meas$. For such a node defined by Pauli $P$, the simplest version of NodeCost is given by \albert{Let's define the Sup function in the section on Paulis}
\begin{align}
\text{NodeCost}(n(P)) = \text{Sup}(P) - 1.
\end{align}
As argued in Ref. \cite{Schmitz2021}, this is the minimum number of TQE gates required to reduce the node to support one, and thus able to be pushed to the circuit.

Factor nodes are those defined by two anti-commuting Pauli operators. It is advantageous to understand factor nodes as defining an effective qubit (partial dimension-2 factorization of the Hilbert space) by defining an effective Z and effective X, much like the rows of the Pauli frame. These nodes include $\Rot^2$, $\Prep$, and the interpretation of a row in the Pauli frame as its own node-type which we refer to as a \emph{local frame}. 
Defining the cost of a factor node requires more machinery. To understand the minimum number of TQE gates to reduce such nodes, i.e. reduce the effective qubit to an actual one, we introduce the \emph{local support matrix} for any anti-commuting pair $(P, Q)$, and any qubit $i$ as
\begin{align}
\text{Sup}_i(P, Q) =
\begin{pmatrix}
    \lambda(P, X_i) & \lambda(P, Z_i)  \\
     \lambda(Q, X_i) & \lambda(Q, Z_i) 
\end{pmatrix},
\end{align}
and the determinant (mod 2) of the local support matrix as the \emph{local determinant}. 
For any factor node whose local determinant is 1 on qubit $i$, we say that node has \emph{strong support} on qubit $i$ and likewise if the local support matrix is not zero, but has zero determinant, we say that node has \emph{weak support} on qubit $i$. We argue in \albert{sup mat; longer version?}, that for any factor node, the sum over all local determinants must be $1 \mod 2$. We also argue for a given factor node, there exists six TQE gates for any pair of qubits with strong support, such that under conjugation, the support is reduced to weak support on both qubits, and for any qubit pair with one strong support and one weak support, there is exactly one TQE gate which will reduce the weak support to no support \albert{summarize these results in a table?}\footnote{We note here that there does exists cases where a TQE gate can reduce two qubits with weak support to one qubit with weak support, but it is not guaranteed in all cases, so we ignore this possibility without violating the promises made by the search functions.}. With these results, we see that the process of reducing a Pauli factor node is the process of reducing all strong support to a single qubit (which will constitute the final qubit on which the node is reduced to) and reducing all weak support (included those which were formerly strong support) to no support. As such, we define the basic search function NodeCost for a factor node as
\begin{align}
\text{NodeCost}(n(P,Q)) =& \left(\sum_i \det\text{Sup}_i(P,Q) - 1\right)/2
\\ &+ \sum_i \left[\text{Sup}_i(P,Q) \neq 0\right] - 1
\end{align}
The first term represents the number of TQE gates to reduce strong support to one and the second term (including the minus 1) is the number of TQE gates to reduce all weak support.

From the NodeCost function, we see that the ReduceNode function simply has to produce all gates which reduce support or support type on any one of the supported qubits by one. Such methods are described explicitly in the \albert{sup mat; longer version?}.

The final two search function--in their most basic form--are straight forward. GateCost is the average change in the NodeCost function for all remaining nodes. We use the average change as opposed to the average absolute cost as this is cheaper to compute in practice, as described in the \albert{sup mat; longer version?}. Likewise, addGate directly adds the gate as passed to the circuit and produces the equivalent change to the PoPR graph, be that removal of a reduced node, or conjugation by the inverse of the passed Clifford gate.

All other versions of the search functions are variations on the basic version. In the case of the Intel Quantum SDK, other considerations include:
\begin{itemize}
    \item a ``schedule'' search which maintains an approximate ASAP scheduling of the circuit. The GateCost function then includes a circuit depth credit as described in Ref. \cite{Schmitz2021} proportional to the difference between the leading time edge of the circuit and the time at which the passed gate might be scheduled.
    
    \item a ``native gate'' search whereby the backend native gate set is known and utilized to reduce the circuit cost at synthesis. In the case of the the Intel Quantum SDK, the gate set of interest is \{CZ, RXY, MeasZ, and PrepZ\}. As such, we want to avoid the generation of RZ gates, and use the know decomposition of non-native gates, especially TQE gates, at the point of synthesis. This requires a modification primarily to the search function AddGate. When a TQE gate is passed to the function, it uses an asymmetric equivalent\footnote{Equivalence is with respects to the Pauli Frame equivalence classes of equally-entangled frames; see Ref. \cite{Schmitz2021}.} where the last gate in the decomposition is a CZ. These asymmetric equivalents are show in Fig. \albert{fig}. The asymmetric equivalent will provide the same reduction for NodeCost, but also guarantees that for the sake of reducing multi-qubit rotation nodes, the node will never be pushed to the circuit as an RZ. To see this, suppose it were pushed to the circuit as an RZ. Then this new gate would commute with the CZ coming from the last asymmetric TQE gate and as such, the rotation could have been effectively converted to the circuit without that TQE gate. Though this reduces the chances that synthesis results in an RZ gate, it doesn't remove the possibility entirely. So when an RZ is passed to AddGate, the following decomposition is used \albert{need a consensus on gate formatting}:
    \begin{align}
    \RZ_q(\theta) = \X_q \RXY_q(\pi, -\theta/2)
    \end{align}
    where the RXY gate is pushed to the circuit and the X is pushed to the graph to be eventually absorbed by the terminating frame. Similarly, when a gate-equivalent Meas or Prep is passed to AddGate which is not in the Z basis, only half of the appropriate Clifford conjugation along with the MeasZ or PrepZ gate is pushed to the circuit while the second half of the conjugation is pushed to the graph.

    \item GateCost also includes a cost penalty for the action of the gate on the terminating frame. An average change in cost over the rows of the Pauli frame--interpreted as local frame nodes--is added to penalize the generation of costly Pauli frames to synthesize (see below).

    \item An alternative modification on any set of search functions can be used to adapt ultra-greedy search to the task of a \emph{stabilizer search} which produces an efficient circuit to simultaneously measure any mutually commuting set of Pauli operators. The description of the stabilizer search algorithm as implemented by ultra-greedy search is the contents of the \albert{companion paper}.
    
    \item \albert{Should we include this bullet?} Future plans include search functions which are adapted to limited connectivity, inexact and noisy gates and additional refinements to GateCost including a weighting of the node averaging based on distance in the partial ordering of the PoPR graph.  
\end{itemize}

\subsubsection{Adaptation of Ultra-Greedy Search for Clifford Synthesis}

After the synthesis of the non-Clifford nodes, the returned outcome of Algorithm \ref{algo:greedy}, $C:G'$, has only the terminating frame left to synthesize into gates. If the quantum state is released as discussed in Section \albert{probably \ref{sec:opts}}, then the terminating frame can be discarded. However, if the state is not released, we must produce an equivalent circuit to complete the synthesis process. Though other methods exist for doing so as in Refs. \cite{Aaronson2004} \albert{more to add...}, we leverage the ultra greedy search for this task because doing so will automatically take into account all the considerations and refinements one has for the synthesis of the non-Clifford nodes. As such, Pauli frame synthesis is described exactly as that of Algorithm \ref{algo:greedy} with the only distinction being that the rows of the Pauli frame are re-interpreted as a set of mutually independent local-frame factor nodes, where the gate-equivalent of a fully reduced local frame is the single-qubit Clifford it represents. we are also guaranteed that when one local frame is reduced, it is independent of all other local frames (i.e. single-qubit operators for the real qubit the local frame is reduced to, cannot appear in any other local frame), as the conjugation by Clifford gates can not change the commutativity relations between the local frames. As such, no TQE gates on that real qubit will be returned by the search functions for the remainder of the synthesis. The only remaining consideration is whether the local frame is reduced to the same or a different qubit than its original row index. When different, this represents the fact that the overall process has swapped qubit indices. In some cases, and as is the case in the current implementation, this swapping is considered free as it can be implemented virtually. However, there may be circumstances where this qubit swapping must be performed by gates, so future version may include the cost of qubit swapping. 

\subsubsection{Time Complexity of the Ultra-Greedy Search Algorithm}

As argued and demonstrated in Ref. \cite{Schmitz2021}, the time-complexity of the ultra-greedy search algorithm is rough $\mathcal{O}(N^3|G|^2)$ in the case where all nodes are independent and we expect roughly the same scaling or better in the general case. This scaling can be dramatically improved (or made worse) based on the complexity of implementing the search functions where the primary driver of that cost is often GateCost. For example, there exists ways to decrease the time complexity for ultra-greedy search with the basic search functions by a factor of $N$ but at the cost of an increase in memory of $\mathcal{O}(N^2)$. Likewise, limiting the connectivity may or may not reduce the complexity due to the scaling of the number of possible TQE gates from $\mathcal{O}(N^2)$ to $\mathcal{O}(N)$ in realistic qubit topologies. However, that may be offset by other costs. More on this in future work. Either way, the GateCost function complexity can always be reduced (leaving a floor for ultra greedy search of $\Omega(N|G|)$) without affecting the two most important properties, algorithm termination and outcome correctness, albeit at the cost of circuit performance. More work is needed to understand this trade-off. 
